Fast Footstep Planning on Uneven Terrain Using Deep Sequential Models

One of the fundamental challenges in realizing the potential of legged robots is generating plans to traverse challenging terrains. Control actions must be carefully selected so the robot will not crash or slip. The high dimensionality of the joint space makes directly planning low-level actions from onboard perception difficult, and control stacks that do not consider the low-level mechanisms of the robot in planning are ill-suited to handle fine-grained obstacles. One method for dealing with this is selecting footstep locations based on terrain characteristics. However, incorporating robot dynamics into footstep planning requires significant computation, much more than in the quasi-static case. In this work, we present an LSTM-based planning framework that learns probability distributions over likely footstep locations using both terrain lookahead and the robot's dynamics, and leverages the LSTM's sequential nature to find footsteps in linear time. Our framework can also be used as a module to speed up sampling-based planners. We validate our approach on a simulated one-legged hopper over a variety of uneven terrains.

==> related_works.tex <==
Methods that do not make use of learning often are based on solving either graph search or optimization problems. 

Section on learned footstep planning:

The non-convex and noncontinuous nature of footstep planning has spurred researchers to investigate learning based approaches to solve this problem. Common approaches include the use of Reinforcement Learning (RL) with a variety of models ranging from a one legged hopper to a full quadruped. Most of these approaches plan footsteps over a relatively short horizon [RLOC][DeepGait][DeepQ Stepper], and have heuristic terms that penalize footstep placements close to designer-specified features in the terrain. VAEs have also been explored to deal with the multimodality problem of footstep planning [Expert Skill-space for replanning]. 

Updated section on optimization:

Other optimization based approaches incorporate terrain knowledge and simplify the problem by making convex approximations to the true underlying dynamics of the system. [Ponton] 

In addition the SLIP model is often used to plan trajectories for higher-dimensional robots such as Cassie. This makes SLIP an attractive model to target for such a learning system, where a large number of offline experiences can be cached in a shorter amount of time, where even offline planners for full-dimensional systems on varied terrains can take minutes to complete for a single problem [TODO: find a citation for this], making the generation of offline training data difficult (is there a logical inconsistency here between dinging other papers for making approximations while also using the SLIP model?).



Updated section on the SLIP model:
For our work, we consider the classic Spring Loaded Inverted Pendulum (SLIP) hopper \cite{schwind_spring_1998}: a one legged machine modeled as a massless, spring-loaded leg and foot attached to a point mass body. This model is often used as a template \cite{full_templates_1999} to plan trajectories of higher degree of freedom robots such as bipeds and quadrupeds [TODO: citations for this].

The SLIP hopper is a hybrid system with two modes. When the hopper is in the \textit{flight} mode, the foot is not touching the ground and the only force experienced by the body is gravity. When the hopper is in the \textit{stance} mode, the foot is in contact with the ground and the body experiences gravity and a spring force acting through the leg. The instantaneous transition from stance to flight is referred to as \textit{liftoff}, and the transition from flight to stance is \textit{touchdown}. The angle of the leg can be varied prior to each touchdown phase to produce a continuous hopping behavior. 

\subsection{Planar SLIP Model}
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/SLIP_trajectory.png}
    \caption{A typical SLIP hopper trajectory}
    \label{fig:slip_traj}
\end{figure}

We first consider the passive SLIP hopper operating only in the sagittal plane. For this formulation, the total energy of the system cannot be changed by actuating the spring. The state space in flight phase consists of the 2D center of mass coordinates, 2D foot coordinates, and 2D center of mass velocity. Because the body and foot are connected by the leg, and no other force acts on the foot, the velocity of the foot is equal to that of the body. 

The passive, sagittal plane SLIP model has one degree of freedom: the angle of the leg with respect to the ground, applied during flight phase. Because the leg is massless, we assume that the leg angle can be changed instantaneously. The control input is applied at the apex of flight, where the vertical velocity is 0, and will affect the body's trajectory during the following stance phase by controlling the tradeoff between apex height and forward velocity. The touchdown transition occurs when the foot makes contact with the ground. 

In the stance phase, the foot position remains fixed (provided the leg angle remains within the friction cone) while the body pivots around it. Stance lasts as long as the spring is compressed, and liftoff occurs when the leg reaches full extension: $\sqrt{\hat{x}^2 + \hat{z}^2} = L$. A typical trajectory for the SLIP hopper is shown in Figure \ref{fig:slip_traj}. For the full dynamical equations, we refer the reader to \citet{carver_lateral_2009}, whose formulation we used for this work. 

An important property of the SLIP model is that there is no closed form solution for the stance phase dynamics, requiring either an approximation or explicit forward integration in order to calculate the next state after applying a control input \cite{piovan_enforced_2012}. 

\subsection{Failure Cases} \label{sec:failures}
Although the passive SLIP models are relatively simplistic, there are a number of kinematic and dynamic factors that make planning for the SLIP hopper nontrivial over broken terrain. There are a few different ways in which the hopper can crash. The first is the standard kinematic case where the body collides with the terrain, or the foot collides with a vertical surface (although this is technically a friction cone violation, we consider it as collision). Second, the leg angle can exit the friction cone during stance phase, causing the foot to slip. Third, if the hopper's apex height is too high above the terrain, the spring will fully compress during touchdown and will bottom-out, also causing a crash. Finally, because the energy of the passive SLIP model is fixed, there is an inverse relationship between the apex velocity $\dot{x}$ and apex height $z$. If the hopper travels too fast, the apex height will not be sufficient for the foot to swing to its position for the next step, causing the robot to "trip" on the ground.

A functional planner must be able to successfully avoid all of these scenarios while also accounting for the robot's current dynamic state. The intersection of the kinematically feasible and dynamically reachable sets of states is not immediately apparent just by analyzing the terrain. Therefore, when planning a trajectory, one must either precompute a set of feasible motion primitives for varying terrains, perform search by sweeping over control inputs and simulating the dynamics, or solve a nonconvex optimization problem. 

